Unsupervised Story Discovery from Continuous News Streams via Scalable Thematic Embedding

Unsupervised discovery of stories with correlated news articles in real-time helps people digest massive news streams without expensive human annotations. A common approach of the existing studies for unsupervised online story discovery is to represent news articles with symbolic- or graph-based embedding and incrementally cluster them into stories. Recent large language models are expected to improve the embedding further, but a straightforward adoption of the models by indiscriminately encoding all information in articles is ineffective to deal with text-rich and evolving news streams. In this work, we propose a novel thematic embedding with an off-the-shelf pretrained sentence encoder to dynamically represent articles and stories by considering their shared temporal themes. To realize the idea for unsupervised online story discovery, a scalable framework USTORY is introduced with two main techniques, theme- and time-aware dynamic embedding and novelty-aware adaptive clustering, fueled by lightweight story summaries. A thorough evaluation with real news data sets demonstrates that USTORY achieves higher story discovery performances than baselines while being robust and scalable to various streaming settings.

==> Tables/Ablation.tex <==
\begin{table}[h]
\caption{Ablation study accuracy.}
\small
\begin{tabular}{lccc} 
\toprule
                                       & Newsfeed14 & WCEP18 & WCEP19 \\ \hline
\algname{}                             & \textbf{0.789}      & \textbf{0.808}  & \textbf{0.825}  \\
\algname{} (w/o theme-aware)           & 0.767               & 0.771           & 0.784  \\
\algname{} (w/o time-aware)            & 0.780               & 0.802           & 0.817  \\
\algname{} (w/o theme-/time-aware)     & 0.752               & 0.756           & 0.771  \\ 
\bottomrule
\end{tabular}
\end{table}

==> Tables/OverallAccuracy_bak.tex <==
\small
\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule
                & \multicolumn{5}{c}{News14}        & \multicolumn{5}{c}{WCEP18}            & \multicolumn{5}{c}{WCEP19}            \\
                & $B^{3}$-P     & $B^{3}$-R     & $B^{3}$-F1    & AMI   & ARI   & $B^{3}$-P     & $B^{3}$-R     & $B^{3}$-F1    & AMI   
                & ARI   & $B^{3}$-P     & $B^{3}$-R     & $B^{3}$-F1    & AMI   & ARI   \\ \hline
ConStream            & 0.213          & \textbf{0.937} & 0.314          & 0.128          & 0.069          & 0.341          & 0.581          & 0.408          & 0.444          & 0.222          & 0.349          & 0.542          & 0.400            & 0.497          & 0.292          \\
\emph{\quad variant with SenT5}         & 0.271          & 0.890          & 0.388          & 0.282          & 0.139          & 0.887 & 0.593          & 0.707          & 0.788          & 0.660          & 0.902 & 0.587         & 0.705         & 0.793          & 0.669          \\

\emph{\quad variant with SenRB}         & 0.334          & 0.794          & 0.434          & 0.413          & 0.276          & \textbf{0.910} & 0.575          & 0.701          & 0.784          & 0.657          & \textbf{0.924} & 0.576          & 0.704          & 0.795          & 0.667          \\ \hdashline
NewsLens             & 0.357          & 0.838           & 0.481          & 0.309          & 0.077          & 0.422          & 0.738          & 0.527          & 0.490          & 0.117          & 0.469         & 0.711          & 0.554          & 0.529          & 0.141          \\
NewsLens*-SenT5          & 0.571          & 0.724         & 0.622          & 0.539          & 0.261          & 0.666         & 0.605          & 0.630          & 0.688          & 0.332          & 0.690          & 0.617          & 0.649          & 0.711         & 0.370          \\
NewsLens*-SenRB          & 0.656          & 0.898          & 0.749          & 0.718          & 0.564          & 0.723          & 0.823          & 0.767          & 0.823          & 0.631          & 0.753          & 0.824          & 0.784          & 0.837          & 0.664          \\ \hdashline
Miranda              & 0.727          & 0.722          & 0.706          & 0.726          & 0.572          & 0.643          & 0.769          & 0.694          & 0.786          & 0.571          & 0.647          & 0.769          & 0.698          & 0.791          & 0.574          \\
Miranda*-SenT5           & 0.784 & 0.712           & 0.732          & 0.753          & 0.617          & 0.729          & 0.699          & 0.710          & 0.798           & 0.629          & 0.749           & 0.692          & 0.717          & 0.805          & 0.644          \\
Miranda*-SenRB           & \textbf{0.788} & 0.770           & 0.764          & 0.785          & 0.648          & 0.726          & 0.796          & 0.751          & 0.835          & 0.656          & 0.730           & 0.804          & 0.759          & 0.837          & 0.657          \\ \hdashline
Staykovski              & 0.618          & 0.770           & 0.669          & 0.602          & 0.358          & 0.729          & 0.672          & 0.697          & 0.759          & 0.487          & 0.737          & 0.672          & 0.701          & 0.765          & 0.487          \\
Staykovski*-SenT5           & 0.601          & 0.831          & 0.684           & 0.631          & 0.415          & 0.674          & 0.818 & 0.735          & 0.798          &  0.582          & 0.613          & \textbf{0.846}          & 0.704          & 0.782           & 0.537           \\ 
Staykovski*-SenRB           & 0.658          & 0.899          & 0.750           & 0.720           & 0.567          & 0.696          & \textbf{0.833} & 0.754          & 0.824          & 0.642          & 0.711          & 0.829          & 0.762          & 0.830           & 0.660           \\ \hline
\textbf{\algname{}-SenT5}                & 0.734          & 0.801          & 0.751 & 0.763 & 0.638 & 0.758          & 0.812          & 0.780 & 0.846 & 0.694 & 0.789         &  0.814 &  0.799 & 0.861  & 0.733 \\
\textbf{\algname{}-SenRB}                & 0.785          & 0.821          & \textbf{0.789} & \textbf{0.812} & \textbf{0.699} & 0.796          & 0.830          & \textbf{0.810} & \textbf{0.871} & \textbf{0.739} & 0.816          & 0.838 & \textbf{0.825} & \textbf{0.880} & \textbf{0.765} \\ 
\textbf{\quad w/o time-aware}                & 0.781          & 0.807          & 0.780 & 0.801 & 0.682 & 0.794          & 0.813          & 0.801 & 0.864 & 0.736 & 0.818          & 0.820 & 0.817 & 0.875 & 0.760 \\ 
\textbf{\quad w/o theme-aware}                & 0.736          & 0.831          & 0.767 & 0.792 & 0.665 & 0.730         & 0.824          & 0.771 & 0.842 & 0.679 &  0.750        &  0.842  & 0.790  &0.856 & 0.703 \\ 
\textbf{\quad w/o both}                & 0.736           & 0.800          & 0.752 & 0.777 & 0.651 & 0.734          & 0.780          & 0.753 & 0.826 & 0.677 & 0.767         & 0.777 & 0.770 & 0.843 & 0.709 \\ 
\bottomrule
\end{tabular}

==> Tables/OverallAccuracy_bak2.tex <==

\begin{tabular}{c|l|ccc|ccc|ccc}
\toprule
               \multicolumn{2}{c}{} & \multicolumn{3}{c}{News14}        & \multicolumn{3}{c}{WCEP18}            & \multicolumn{3}{c}{WCEP19}            \\
                & & $B^{3}$-F1  & AMI   & ARI   &  $B^{3}$-F1   & AMI   & ARI   &  $B^{3}$-F1  & AMI    & ARI   \\ \hline
\multirow{5}{*}{Baselines} & ConStream            & 0.314          & 0.128          & 0.069              & 0.408          & 0.444          & 0.222               & 0.400            & 0.497          & 0.292          \\ 

& NewsLens                      & 0.481          & 0.309          & 0.077         & 0.527          & 0.490          & 0.117       & 0.554          & 0.529          & 0.141          \\ 

& Miranda                 & 0.706          & 0.726          & 0.572              & 0.694          & 0.786          & 0.571             & 0.698          & 0.791          & 0.574          \\ 

& Staykovski                     & 0.669          & 0.602          & 0.358               & 0.697          & 0.759          & 0.487             & 0.701          & 0.765          & 0.487          \\  
& StoryForest                 & xxx          & xxx          & xxx               & 0.673          & 0.765          & 0.523                 & xxx          & xxx          & xxx          \\  \hdashline

\multirow{4}{*}{
\begin{tabular}[c]{@{}c@{}} PSE-variants of \\  the top baselines \end{tabular}} & Miranda$^{*}$-SenT5                 & 0.732          & 0.753          & 0.617                & 0.710          & 0.798           & 0.629           & 0.717          & 0.805          & 0.644          \\
& Staykovski$^{*}$-SenT5                    & 0.684           & 0.631          & 0.415       & 0.735          & 0.798          &  0.582            & 0.704          & 0.782           & 0.537           \\ 
 & Miranda$^{*}$-SenRB                   & 0.764          & 0.785          & 0.648             & 0.751          & 0.835          & 0.656               & 0.759          & 0.837          & 0.657          \\ 
& Staykovski$^{*}$-SenRB              & 0.750           & 0.720           & 0.567        & 0.754          & 0.824          & 0.642                 & 0.762          & 0.830           & 0.660           \\ \hline

\multirow{3}{*}{Proposed} & \textbf{\algname{}-SenT5}   & \begin{tabular}[c]{@{}c@{}} \textbf{0.751}$^{*}$\\ \footnotesize{($\triangle 6.4,\blacktriangle 2.6$)}\end{tabular} & 0.763 & 0.638        & 0.780 & 0.846 & 0.694 &  0.799 & 0.861  & 0.733 \\
& \textbf{\algname{}-SenRB}           & \begin{tabular}[c]{@{}c@{}} \textbf{0.789}$^{*}$\\ \footnotesize{($\triangle 11.8,\blacktriangle 3.3$)}\end{tabular} & \textbf{0.812} & \textbf{0.699}          & \textbf{0.810} & \textbf{0.871} & \textbf{0.739}& \textbf{0.825} & \textbf{0.880} & \textbf{0.765} \\  \hdashline
\multirow{3}{*}{
\begin{tabular}[c]{@{}c@{}} Variants of \\  \algname{}-SenRB \end{tabular}} & \textbf{\quad w/o time-aware}      & 0.780 & 0.801 & 0.682         & 0.801 & 0.864 & 0.736  & 0.817 & 0.875 & 0.760 \\ 
& \textbf{\quad w/o theme-aware}     & 0.767 & 0.792 & 0.665           & 0.771 & 0.842 & 0.679   & 0.790  &0.856 & 0.703 \\ 
& \textbf{\quad w/o both}               & 0.752 & 0.777 & 0.651           & 0.753 & 0.826 & 0.677  & 0.770 & 0.843 & 0.709 \\ 
\bottomrule
\end{tabular}
